The mercurial Sun at the heart of our solar system

As the powerhouse of our solar system, the Sun's electromagnetic planetary influences appear contradictory. On the one hand, the Sun for aeons emitted radiation which was "just right" for life to evolve in our terrestrial Goldilocks zone, even for such complex organisms as ourselves. On the other, in the dawn of Earth's existence the Sun was far dimmer than today, and yet evidence for early liquid water is written into geology. Now in middle age, the Sun should be a benign object of little interest to society or even astronomers. However, for physical reasons yet to be fully understood, it contains a magnetic machine with a slightly arrhythmic 11 year magnetic heartbeat. Although these variations require merely 0.1% of the solar luminosity, this power floods the solar system with rapidly changing fluxes of photons and particles at energies far above the 0.5eV thermal energy characteristic of the photosphere. Ejected solar plasma carries magnetic fields into space with consequences for planets, the Earth being vulnerable to geomagnetic storms. This chapter discusses some physical reasons why the Sun suffers from such ailments, and examine consequences through time across the solar system. A Leitmotiv of the discussion is that any rotating and convecting star must inevitably generate magnetic "activity" for which the Sun represents the example par excellence.

==> macros.tex <==
\newcommand{\pref}{\protect\ref}
\newcommand{\solrad}{\ifmmode{R}_{\rm S}\else${R}_{\rm S}$\fi}
\newcommand{\solmas}{\ifmmode{M}_{\rm S}\else${M}_{\rm S}$\fi}
\newcommand{\ergu}{$\,$ergs$\,$s$^{-1}$}
\newcommand{\flxu}{\ifmmode{\rm W~m^{-2}}\else W~m$^{-2}$\fi}
\newcommand{\intu}{\ifmmode{\rm W~m^{-2}~sr^{-1}~hz^{-1}}\else 
                   W~m$^{-2}$~sr$^{-1}$~hz^{-1}\fi}
\newcommand{\tintu}{\ifmmode{\rm W~m^{-2}sr^{-1}}\else W~m$^{-2}$~sr$^{-1}$\fi}
\newcommand{\velu}{$\,$km$\,$s$^{-1}$}
\newcommand{\dynu}{$\,$dyn$\,$cm$^{-2}$}
\newcommand{\wave}{\ifmmode{\lambda} \else$\lambda$\fi}
\newcommand{\freq}{\omega}
%\newcommand{\freq}{\nu}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\let\la=\lesssim
\def\ion#1#2{#1$\;${\rm%
      \expandafter\uppercase\expandafter{\romannumeral #2}\ignorespaces}\relax}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% cross, divergence, grad, curl operators
%
\renewcommand{\vec}[1]{{\bf #1}}
\newcommand{\matrx}[1]{
    \ifmmode{\underline{\underline {\bf #1}}}
    \else ${\underline{\underline {\bf #1}}}$
    \fi}
\newcommand{\totd}[1]{
    \ifmmode{ {{\partial{#1}}\over {\partial t}} + \vec{v}\cdot\nabla #1}
    \else${ {{\partial{#1}}\over {\partial t}} + \vec{v}\cdot\nabla #1}$
    \fi}    
\newcommand{\cross}{\times}
\newcommand{\divg}{{\rm div\,}}
\newcommand{\grad}{{\bf grad\,}}
\newcommand{\curl}{{\bf curl\,}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ord}{\ensuremath{\mathcal O}}
\newcommand{\cond}{\ensuremath \sigma}

% From M. Rempel
%\renewcommand{\vec}[1]{{\bm{#1}}}
\newcommand{\di}{\vec{\nabla}\cdot}
%\renewcommand{\curl}{\vec{\nabla}\times}
%\renewcommand{\grad}{\vec{\nabla}}
\newcommand{\E}{\vec{E}}
\newcommand{\B}{\vec{B}}
\newcommand{\jj}{\vec{j}}
\newcommand{\vv}{\vec{u}}
\newcommand{\eps}{\varepsilon}
\newcommand{\rh}{\rho}
\newcommand{\dd}{\partial}
\newcommand{\DD}{\Delta}
\newcommand{\dt}{\partial t}
\newcommand{\Dt}{\Delta t}
\newcommand{\avr}[1]{\overline{#1}}
\newcommand{\pr}[1]{{#1}^{\prime}}
\newcommand{\degr}{^\circ}
\newcommand{\emf}{\avr{\vec{\mathcal{E}}}}

\newcommand{\dbdt}{\ensuremath {{ {\partial \vec{B}}\over {\partial t} } }}
\newcommand{\dedt}{\ensuremath {{1 \over{2 \mu_0}} { {\partial B^2 } \over {\partial t} } }}

\newcommand{\ssr}{Space Sci. Rev.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% stacked math symbols
%% macro by Louis Strous, after char.mac Skumanich Soesterberg 
%% usage: \mathstacksym\newsymbol{upper_symbol}{lower_symbol}
%%                               {upper_height}{lower_depth}
\def\mathstacksym#1#2#3#4#5{\def#1{\mathrel{\hbox to 0pt{\lower {#3}\hss} \raise #4\hbox{#2}}}}

\mathstacksym\lta{$<$}{$\sim$}{1.5pt}{3.5pt} % less than approximately
\mathstacksym\gta{$>$}{$\sim$}{1.5pt}{3.5pt} % greater than approximately
\mathstacksym\lrarrow{$\leftarrow$}{$\rightarrow$}{2pt}{1pt} % equilibrium
\mathstacksym\lessgreat{$>$}{$<$}{3pt}{3pt} %% less or greater

%%%%%%%%%%%%%%%%%%%%  END OF FILE RRMACROS.TEX  %%%%%%%%%%%%%%%%%%%%%%%%%%%


